VLUE: A New Benchmark and Multi-task Knowledge Transfer Learning for Vietnamese Natural Language Understanding

The success of Natural Language Understanding (NLU) benchmarks in various languages, such as GLUE for English, CLUE for Chinese, KLUE for Korean, and IndoNLU for Indonesian, has facilitated the evaluation of new NLU models across a wide range of tasks. To establish a standardized set of benchmarks for Vietnamese NLU, we introduce the first Vietnamese Language Understanding Evaluation (VLUE) benchmark. The VLUE benchmark encompasses five datasets covering different NLU tasks, including text classification, span extraction, and natural language understanding. To provide an insightful overview of the current state of Vietnamese NLU, we then evaluate seven state-of-the-art pre-trained models, including both multilingual and Vietnamese monolingual models, on our proposed VLUE benchmark. Furthermore, we present CafeBERT, a new state-of-the-art pre-trained model that achieves superior results across all tasks in the VLUE benchmark. Our model combines the proficiency of a multilingual pre-trained model with Vietnamese linguistic knowledge. CafeBERT is developed based on the XLM-RoBERTa model, with an additional pretraining step utilizing a significant amount of Vietnamese textual data to enhance its adaptation to the Vietnamese language. For the purpose of future research, CafeBERT is made publicly available for research purposes.

==> figures/analysis_performance.tex <==

\begin{figure*}[!ht]
\centering
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        width  = 1*\textwidth,
        height = 8cm,
        major x tick style = transparent,
        ybar=1*\pgflinewidth,
        axis x line*=bottom,
        bar width=15pt,
        ymajorgrids = true,
        ylabel = {F1-score},
        symbolic x coords={UIT-ViQuAD 2.0, ViNLI, VSMEC, ViHOS, NIIVTB POS},
        xtick = data,
        ymin=0,
        % xticklabel style={rotate=45},
        nodes near coords,
        enlarge x limits=0.2,
        every node near coord/.append style={rotate=90, anchor=west},
        %ymin=0,
        scaled y ticks = false,
        % legend cell align=top,
        % legend style={
        %         at={(1,1.05)},
        %         anchor=south east
        % }
        legend style={
                    at={(0.0,-0.15)},
                    anchor=north west,
                    legend columns=-1,
                    /tikz/every even column/.append style={column sep=1.0cm}
                        }
    ]
    
        \addplot coordinates {(UIT-ViQuAD 2.0,94.78) (ViNLI,96.67) (VSMEC, 92.04) (ViHOS, 94.35) (NIIVTB POS, 96.67)};
        % \addplot[pattern=dots] coordinates {(UIT-ViQuAD 2.0,94.78) (ViNLI,96.67) (VSMEC, 92.04) (ViHOS, 94.35) (NIIVTB POS, 96.67)}; [style={blue,fill=bblue,mark=black}]
             
        \addplot coordinates {(UIT-ViQuAD 2.0,84.22) (ViNLI,79.80) (VSMEC,67.48) (ViHOS, 90.19) (NIIVTB POS, 96.64)};
        % \addplot[pattern=north east lines] coordinates {(UIT-ViQuAD 2.0,84.22) (ViNLI,79.80) (VSMEC,67.48) (ViHOS, 90.19) (NIIVTB POS, 96.64)};

        \addplot coordinates {(UIT-ViQuAD 2.0, 64.42) (ViNLI,57.35) (VSMEC, 45.57) (ViHOS, 71.42) (NIIVTB POS, 91.63)};
        % \addplot[pattern=grid] coordinates {(UIT-ViQuAD 2.0, 64.42) (ViNLI,57.35) (VSMEC, 45.57) (ViHOS, 71.42) (NIIVTB POS, 91.63)};

        \addplot coordinates {(UIT-ViQuAD 2.0, 46.96) (ViNLI,19.08) (VSMEC, 14.56) (ViHOS, 42.52) (NIIVTB POS, 85.99)};
        % \addplot[pattern=horizontal lines] coordinates {(UIT-ViQuAD 2.0, 46.96) (ViNLI,19.08) (VSMEC, 14.56) (ViHOS, 42.52) (NIIVTB POS, 85.99)};
        \legend{Set1, Set2, Set3, Set4}
    \end{axis}
\end{tikzpicture}
    \caption{Performance of the CafeBERT pre-trainned model on subsets of all tasks in the VLUE benchmark.}\label{lbl:performance_4set}
\end{figure*}

==> tables/num_samples_subset.tex <==
\begin{table}[]
\centering
\begin{tabular}{lcccc}
\hline
                        & \multicolumn{1}{l}{\textbf{set1}} & \multicolumn{1}{l}{\textbf{set2}} & \multicolumn{1}{l}{\textbf{set3}} & \multicolumn{1}{l}{\textbf{set4}} \\ \hline
\textbf{UIT-ViQuAD 2.0} & 2,091                              & 530                               & 355                               & 845                               \\
\textbf{ViNLI}          & 2,271                              & 301                               & 142                               & 277                               \\
\textbf{VSMEC}          & 374                               & 55                                & 71                                & 186                               \\
\textbf{ViHOS}          & 210                               & 400                               & 17                                & 478                               \\
\textbf{NIIVTB POS}     & 754                               & 289                               & 167                               & 748                               \\ \hline
\end{tabular}
\caption{The number of samples of each subset of each dataset in the VLUE benchmark.\label{tab:num_samples_subset}}
\end{table}

==> tables/performance_dev.tex <==
\begin{table*}[]
\centering
\begin{tabular}{lccccc}
\hline
                     & \textbf{UIT-ViQuAD 2.0} & \textbf{ViNLI} & \textbf{VSMEC} & \textbf{ViHOS} & \textbf{NIIVTN POS} \\ \hline
\textbf{PhoBERT$_{large}$}     & 73.79                   & 80.81          & \textbf{60.93}          & 76.11          & 82.00               \\
\textbf{XLM-Roberta$_{large}$} & 78.15                   & 86.90          & 57.02          & 77.13          & 89.98               \\
\textbf{CafeBERT}    & \textbf{79.75}                   & \textbf{86.98}          & 60.32          & \textbf{77.72}          & \textbf{90.87}               \\ \hline
\end{tabular}
\caption{\label{tab:performance_dev} Performance of the three models on the VLUE benchmark. We use F1 score to evaluate all tasks on the dev sets.}
\end{table*}
